Quantum isometry groups

This thesis contains the formulation and computation of quantum isometry groups.

==> thanks.tex <==
\chapter{Acknowledgement}




==> title.tex <==

%\pagestyle{empty} 
\vspace*{1cm} 
\begin{center} 
\begin{large} 
\textbf{QUANTUM  ISOMETRY  GROUPS\\} 
\end{large} 
\end{center} 

\vspace{3cm} 

\begin{center} 
\begin{large} 
\textbf{JYOTISHMAN BHOWMICK\\} 
\end{large} 
\end{center} 

\vspace{4cm} 
\begin{figure}[h] 
\begin{center} 
%\includegraphics[width=4cm]{logo.pdf} 
\end{center} 
\end{figure} 
\vspace{2cm} 

\begin{center} 
\begin{large} 
\textbf{INDIAN STATISTICAL INSTITUTE, KOLKATA\\ 
2009} 
\end{large} 
\end{center} 

\cleardoublepage 

%\pagestyle{empty} 
%\vspace*{1cm} 
\begin{center} 
\begin{large} 
\textbf{QUANTUM  ISOMETRY  GROUPS\\} 
\end{large} 
\end{center} 

\vspace{2cm} 

\begin{center} 
\begin{large} 
\textbf{JYOTISHMAN BHOWMICK\\} 
\end{large} 
\end{center} 

\vspace{4cm} 
\begin{center} 
\textbf{Thesis submitted to the Indian Statistical Institute\\ 
in partial fulfilment of the requirements\\ 
for the award of 
the degree of\\ 
Doctor of Philosophy.\\ 
 2009}\\
\textbf{Thesis Advisor: Debashish Goswami}
\end{center} 

\vspace{1cm} 
\begin{figure}[h] 
\begin{center} 
%\includegraphics[width=2cm]{ISI.eps} 
\end{center} 
\end{figure} 
\vspace{1cm} 

\begin{center} 
\begin{large} 
\textbf{Indian Statistical Institute\\ 
203, B.T. Road, Kolkata, India.} 
\end{large} 
\end{center} 

